Relational Network Verification

Relational network verification is a new approach to validating network changes. In contrast to traditional network verification, which analyzes specifications for a single network snapshot, relational network verification analyzes specifications concerning two network snapshots (e.g., pre- and post-change snapshots) and captures their similarities and differences. Relational change specifications are compact and precise because they specify the flows or paths that change between snapshots and then simply mandate that other behaviors of the network "stay the same", without enumerating them. To achieve similar guarantees, single-snapshot specifications need to enumerate all flow and path behaviors that are not expected to change, so we can check that nothing has accidentally changed. Thus, precise single-snapshot specifications are proportional to network size, which makes them impractical to generate for many real-world networks. To demonstrate the value of relational reasoning, we develop a high-level relational specification language and a tool called Rela to validate network changes. Rela first compiles input specifications and network snapshot representations to finite state transducers. It then checks compliance using decision procedures for automaton equivalence. Our experiments using data on complex changes to a global backbone (with over 10^3 routers) find that Rela specifications need fewer than 10 terms for 93% of them and it validates 80% of them within 20 minutes.

==> sections/obsolete.tex <==
\begin{figure*}
    \begin{subfigure}{.33\textwidth}
        \centering
        \begin{tikzpicture}
          % First circle
          \draw (0,0) circle [radius=.6cm];
          % Second circle
          \draw (2.5,0) circle [radius=.6cm];
          % Arrow
          \draw[->] (.8,0) -- (1.7,0);
      
          % Labeling the circles
          \node at (0,0) {Old};
          \node at (2.5,0) {New};
          %\node at (0,1) {$\mathrm{Old} \vDash P_{pre}$};
          \node at (2.5,1) {$\mathrm{New} \vDash P$ ?};

        \end{tikzpicture}
        \caption{Traditional verification.}
        \label{fig:traditional_paradigm}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
        \centering
        \begin{tikzpicture}
            % First circle
            \draw (0,0) circle [radius=.6cm];

            % Second circle
            \draw (.4,0) circle [radius=.6cm];

            % Labeling the circles
            \node at (0.2,1) {$\left( \mathrm{Old} \oplus \mathrm{New} \right) \vDash P_{diff}$ ?};
            \node at (-0.38,0) {$-$};
            \node at (0.78,0) {$+$};

            % Overlapping area
            %\begin{scope}
            %  \clip (0,0) circle [radius=.6cm];
            %  \fill (.4,0) circle [radius=.6cm];
            %\end{scope}

        \end{tikzpicture}
        \caption{Differential verification.}
        \label{fig:differential_paradigm}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
        \centering
        \begin{tikzpicture}
          % First circle
          \draw (0,0) circle [radius=.6cm];
          % Second circle
          \draw (2.5,0) circle [radius=.6cm];
          % Arrow
          \draw[<->] (.8,0) -- (1.7,0);
      
          % Labeling the circles
          \node at (0,0) {Old};
          \node at (2.5,0) {New};
          \node at (1.25,1) {$\left( \mathrm{Old}, \mathrm{New} \right) \vDash P_{rel}$ ?};

        \end{tikzpicture}
        \caption{Relational verification.}
    \end{subfigure}
    \caption{Different paradigms of network change verification.}
    \label{fig:paradigms}
\end{figure*}

\section{Motivation}

%\brief{Goals of this subsection:}

%\brief{- To acknowledge and explain how past dataplane verification efforts work in general (ie: they answer questions of the form "New-Network satisfies Spec"  -- ie, there's one network, the new one, and one spec, which is typically a set of paths)}
%- To remind readers that regular expressions are an example of a specification language that has been used before in traditional networking (eg in NetKAT).  
%- To familiarize readers with path-based specs based on regexps.
%\brief{- To introduce a concrete network and examples that can be elaborated on/extended later.}
%\brief{- To explain the problem - why traditional verification techniques aren't enough.}

%\brief{Existing network change validations systems checks \textit{absolute properties}, \IE, whether the  network state after change (post-state) behaves as intended.}

%\brief{Writing change specifications in this paradigm is challenging for two reasons.}

%Wait, why do people not just use HSA. If they did so, they just need to write down ...

%WHen you change, it's not a new network. What's important is that you don't screw up most part of the network.

%People may not know all parts of the network

%\brief{First, correctness. The absolute properties need to be written using low-level test primitives, such as route inspection tests or reachability tests. Operators need to specify exactly what header space to be checked. This is known to be error-prone. Indeed, we show a network change that lead to outage (\Cref{fig:dns}) due to incorrect specification of header space.}

%\brief{Second, completeness. In this example, users only checks the behavior of flows that are meant to be changed (liveness check). It's never easy to check that the other functionalities of the network should not be broken by the change (safety check), which is arguably even more important.}

     


\begin{figure*}
    \begin{subfigure}{.49\textwidth}  % Subfigure 1
        \centering
        \includegraphics[width=.9\textwidth]{figures/dns_prestate.png}
        \caption{Network state before change.}
        \label{fig:dns_prestate}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}  % Subfigure 2
        \centering
        \includegraphics[width=.9\textwidth]{figures/dns_poststate.png}
        \caption{Network state after change.}
        \label{fig:dns_poststate}
    \end{subfigure}
    \caption{An example network change that leads to an outage. The operators intend to disable traffic from $DC_1$ to region $Y$ (orange arrow), and they implement the change by letting $A$ announce BGP routes learnt from region $Y$ and attaching a tag that indicates other routers to set the route's next hop to ``drop''. Operators tested that $D$ should have BGP routes to $Y$'s assigned IP prefixes and their next hops should be ``drop'', and all tests indeed passed. However, it turned out that the reachability between $DC_1$ and Region $X$'s DNS servers in $DC_2$ (blue arrow) was accidentally broken due to prefix overlap.}
    \label{fig:dns}
\end{figure*}




%Network operators used to write two types of tests to validate the correctness of network changes.
%\begin{itemize}
%    \item Data plane inspection test.
%    \item Reachability test.
%\end{itemize}
%For the first type, operators need to specify a 4-tuple $(r, p, f, v)$, where $r$ is a router in the network, $p$ is a IP prefix, $f$ (for field) is a routing attribute and $v$ is the expected value for the field. For the second type, operators need to specify $(loc, srcIp, dstIp, reach)$, where $loc$ is start location and $reach$ is a Boolean value indicating whether the reachability is supposed to be present.

%These two primitives are low-level, and their parameter spaces are huge. It is tedious and error-prone to validate network change correctness using such tests. Indeed, knowing from the experience in a large cloud provider, the validating process of a network change plan can last several weeks and yet there are still bugs that escaped testing.


%Due to the prevalence of network outages triggered by erroneous network changes, testing and verification techniques \cite{batfish-2023, hoyan, hsa} have been developed and used to find errors in planned network changes prior to their deployment.

%verification tools~\cite{hoyan, jingjing, batfish-2023, rcdc, aws-inspector, deltanet} have been adopted by major cloud providers to find bugs in the implementation of proposed network changes.

%Automated verification has served as key means to prevent outages caused by erroneous network changes. Major cloud providers have integrated verification~\cite{hoyan, jingjing, rcdc} in their network change management workflows. However, as we know from the experience of helping deploy verification for multiple networks, existing verification tools exhibit fundamental flaws in the scenarios of debugging in-production network changes. The verification process requires a lot of human intervention and is thus time-consuming. 
%
%The verification of network changes in industrial settings can last as long as several weeks and yet it can still miss serious bugs.

%The major challenge is to create and maintain a set of faithful specifications of the network. In particular, 1) traditional verification tools assumes the network engineers can have a complete picture of the network being verified, and yet this is impractical for industrial networks. And 2) 

%A lot of human intervention is required, which makes the verification process a time-consuming task, 
%In this section, we highlight two major challenges to enable faithful and ergonomic verification 

%Existing verification tools exhibit fundamental flaws in debugging in-production network changes. Depending on the type of properties used to determine the correctness of a network change, existing tools can be classified as traditional network verification or differential network analysis.

%Every change comes with a risk. When making changes to networks in an industrial setting, network engineers would like to check that 1) the intended change impact is achieved and 2) the other existing functionalities of the network is not broken. However, traditional network verification is designed to reason about a single version of the network regarding its forwarding behavior, which makes both goals above extremely hard to achieve.

%\brief{why it is hard to check that the intended change impact is achieved}
%Many changes are local to only one or a few routers and are conceptually simple, however, small local changes can make huge impact on the end-to-end forwarding behavior. For example, to shut down a core router in our global WAN for maintenance, the configuration change is simple and is limited to only the neighbors of this router. However, since a core router can carry up to O($10^7$) classes of traffic with distinct end-to-end forwarding paths, and all of them are intended to be re-routed when the router is shut down, it is practically impossible for the engineers to specify for each class of traffic how exactly they should be forwarded after the change. The engineers need a more compact way to specify the desired impact of such a change.

%\brief{why it is hard to do safety check}
%It is arguably even more challenging to check whether a change is ``safe''. In a distributed control plane, small local changes may affect the forwarding behavior of seemingly unrelated parts of the network. To ensure that no bad change happened in the network, one needs to check the end-to-end behavior of the entire network. However, many industrial networks have been constructed in an incremental fashion over the course of years. There is no global specification of exactly what such a network should do. So using traditional network verification, which compares the changed network to a spec representing its expected behavior, is not possible.  
%And yet engineers need a way to reliably make changes to such networks.  They need to add, remove, or change functionality in a subpart of the network, typically while preserving most of the network's behavior.

%As we will discuss in this section, Outages happen when the specification was inaccurate such that serious bugs were missed. It is important for the specification to be accurate and complete, otherwise 

%In this section, we discuss the fundamental challenges in verifying the correctness of network changes in an industrial setting.

%Checking how exactly the forwarding behavior should be like before the change and after the change. vs what range of forwarding behavior should be changed and how should it be changed; what range of forwarding behavior should remain the same.






%To ensure the correctness of a network change, one needs to apply verification twice, one for the old version of the network and one for the new version. The problem is, the network

%The pre-conditions usually contains the properties that must be true before a certain change can be made, The post-conditions define the properties of the network that must be true after the change. as illustrated in \Cref{fig:traditional_paradigm}. At the first glance, the major complaint may seem to be redundant computation, because the two versions of the network are vastly similar and yet it takes twice the time to verify them separately. However, as we know from helping deploy network change verification for multiple networks, two more fundamental challenges of this paradigm are that 1) network engineers do not have complete picture of either the Old or the New network and 2) 

%the computational time to verify the forwarding behavior for both networks is in the order of tens of minutes~\cite{hoyan, rcdc}, which is not prominent in the whole workflow which can last several weeks. The actual bottleneck is the excessive requirement of human involvement in 1) writing down the exact properties to verify and 2) understanding the reported counterexamples when verification fails. Let us elaborate.

%To give some concrete numbers, the computational time to verify the reachability properties of a network is in the order of several minutes~\cite{hoyan, rcdc}. As a comparison, even an expert engineer can only audit about 50 classes of network traffic per day, and yet the total number of distinct network traffic carried by our global WAN is in the order of O($10^7$). 



%Traditional network verification is originally designed to verify individual network states. When applied to network changes, the workflow is generally as follows: 1) network engineers create a simulated/emulated replica of the network based on a recent snapshot, denoted as the ``Old'' network. The engineers then 2) apply the change to the replica to derive the after-change network state, denoted as the ``New'' network.  Next, 3) the verification tool is invoked to determine whether the Old meets some pre-conditions and whether the New meets some post-conditions. An illustration of this verification paradigm is shown in \Cref{fig:traditional_paradigm}. 


%The pre-conditions usually contains the properties that must be true before a certain change can be made, \EG, before shutting down a router, the router must exist and be active, and there must be a backup router that can take over the traffic after the previous router is gone. The post-conditions define the properties of the network that must be true after the change, and they are often a combination of:
%\begin{itemize}
    %\item The expected outcome of the change is achieved.
    %\item The existing functionalities of the network are not broken.
%\end{itemize}
%For instance, after applying a change which intends to shut down a router, the first part of post-condition may be that the router must be off; the second part may be that 1) traffic that went through this router before should be re-routed to its backup router and 2) other traffic should not be affected by the change.

%Next, engineers 3) express the expected impact of a change, \IE, the \textit{specifications}. And finally 4) verification tools are invoked to determine whether the change impact matches the specification. If the result is not true, the engineers then go back to debug the change and/or the specification.





%\brief{A real example that leads to an outage.}
%\Cref{fig:dns} shows an example network change simplified from a real network change that caused a significant outage. $R1$, $R2$ and $R3$ are part of the global backbone network that interconnects datacenters and various infrastructure. For simplicity, we only show a DNS server under $R1$ and two datacenters under $R2$ and $R3$ respectively. For interconnectivity, routers announce the prefixes assigned to their attached sub-networks within the backbone using BGP protocol. But they do not announce such learnt routes to further below, instead, they announce an aggregated default route ($0.0.0.0/0$) to attached sub-networks. In this network change, the operators intend to remove inter-region traffic through $R2$ (red arrow), and they implements the change by letting $R2$ announcing BGP routes learnt from foreign regions to its attached subnetwork, with a tag that indicates other routers to set the route's nexthop to drop. Operators tested that $DC2$ should have BGP routes to foreign prefixes and their nexthop should be drop, and all tests indeed passed. However, it turned out that the reachability between $DC2$ and DNS server under $R1$ (blue arrow) was accidentally broken due to prefix overlap.



%\brief{Validating changes is practically hard. Absolute spec is unknown, and even it is known, it will be huge.}
%Every change comes with a risk. When making changes to networks in an industrial setting, network engineers would like to check that 1) the intended change impact is achieved, \IE, liveness, and 2) the other existing functionalities of the network is not broken, \IE, safety. In practice, however, checking liveness and safety for network changes is challenging with traditional network verification. Traditional verification is designed to reason about a single version of the network, and to check a network change, one needs to provide the \textit{specification} of the after-change network. As we will show via a motivating example, in industrial settings, the complete specification of how exactly a network should behave is not known to network engineers. And even if it is known, it will be too verbose to be handled by human. This makes network change verification a tedious task, and yet bugs can still be missed.

\brief{Brief preamble to describe what readers should anticipate from this section}



\subsection{Motivating Example}

\brief{An example network change. lay out the details of the example and what goes wrong}
\Cref{fig:dns} shows a real network change that contains an error that caused a significant outage. For simplicity, we only show related routers and IP prefixes in the figure. Routers $A$, $B$ and $C$ and $D$ are a subpart of a global backbone network that interconnects O(10) of datacenters distributed in different regions. Before the change (\Cref{fig:dns_prestate}), top-tier routers $A$, $B$ and $C$ announce the IP prefixes assigned to their attached sub-networks using BGP protocol, \EG, $C$ announces $10/24$ to $B$, and $B$ announces $10/29$ to $A$. The routes learnt from a neighbor are also re-announced to other neighbors, \EG, $B$ re-announces the route $10/24$ learnt from C to A. To provide connectivity to attached sub-networks, instead of re-announcing all of such learnt routes, the top-tier routers simply announce a default route ($0.0.0.0/0$) to its lower neighbors, such as from $A$ to $D$. As a result, any traffic from $DC_1$ will be forwarded to $A$ by $D$, and it then will be forwarded against the path of BGP route propagation. As shown in the figure, from $DC_1$, traffic destined to $10/29$ will use the path $DC_1 \rightarrow D \rightarrow A \rightarrow B \rightarrow DC_2$, and traffic within $10/24$ but outside of $10/29$ will use the path $DC_1 \rightarrow D \rightarrow A \rightarrow B  \rightarrow C \rightarrow DC_3$. Now it comes the change. In response to a new business regulation, the network engineers intended to disable $DC_1$ from reaching a foreign region $Y$ while preserving other exiting functionalities of the network. In other words, traffic on paths such as the orange arrow should be dropped, and traffic on other paths such as the blue arrow should be preserved. The implementation of the change and its effect is shown in \Cref{fig:dns_poststate}. Based on the knowledge that BGP announcements in the backbone are tagged with their origin region, the engineers changed the configuration of router $A$ such that in addition to the default route, $A$ also re-announced learnt BGP routes to $D$ if they were tagged as from region $Y$ (such as $10/24$). Such announcements were configured with another special tag that indicated other routers to set the route's next hop to be $drop$. Consequently, $D$ would drop any traffic that matches region $Y$'s prefixes. When the change was deployed, it not only dropped the traffic from $DC_1$ to $Y$ that was intended to be dropped, but also accidentally broke the traffic from $DC_1$ to $10/29$, which was used by region $X$'s DNS servers located in $DC_2$. This unexpected effect led to a significant outage.

\brief{state the fundamental barriers to reliable network operation. 1) Incomplete information:  network engineers know only part of the system. 2) Scale: $10^K$ nodes, routes, etc. In this part, do not refer to potential solutions to challenges (ie, don't refer to "traditional verification" or manual inspection), just refer to the fundamental challenges faced by any potential solution.  Description and analysis of solutions comes in the next section.}

\subsection{Three Possible Solutions}

\subsubsection{Single-snapshot verification.}

\brief{Here is how traditional verification works. }

\brief{Here is the problem when we throw it at real network changes. Problem: the absolute spec is not fully available to engineers. Even if they are, they will be huge.}

A main hurdle of traditional verification in such scenarios is that network engineers do not have a complete picture of the network being tested. In the aforementioned change, the engineers should have checked that the traffic from $DC_1$ to $10/29$ are not broken along with traffic to other IPs in $10/24$. However, when implementing and testing this change (which manipulates traffic based on the tags on BGP routes), the engineers were not aware that there was a small overlap between the prefixes for to-be-dropped traffic and to-be-preserved traffic. In fact, they were not even aware of the concrete prefixes for both classes of traffic, as the assignment of IP prefixes was managed by other teams. And this unawareness is not uncommon. Today's industrial networks are tremendously complex in terms of their scale and heterogeneity. They are built incrementally over a course of years, and different parts of them are managed by different teams. As a result, any individual who is asked to test a network change has only partial knowledge of how exactly the network should behave. Any specification about the network provided by such a person is likely to be incomplete or even incorrect. 

A second challenge to specify a network is its verbosity, which makes it impractical to create and maintain full specification of the network even if engineers can have full knowledge to it. Traditional verification models network dataplane properties as either 1) route properties, \EG, router $A$ should have route $10/24$, and the next hop of route $10/24$ on router $A$ should be router $B$, or 2) traffic path properties, \EG, router $D$ should be able to reach $DC_2$ using destination IPs in $10/29$, and such traffic should go through router $A$ and $B$. In the global backbone network that we target to help operate, there are O($10^3$) of routers and an average of O($10^4$) routes on each router. In terms of traffic and their paths, the network carries O($10^9$) classes of traffic with distinct 5-tuples, and even if considering that many traffic share the same paths, there are O($10^7$) equivalent classes of traffic that use different paths. At this scale, concrete specification of either route properties or traffic path properties would be too verbose to be handled by human.

%Recall that to check whether a network change is correct, one needs to ensure that all intended change impact is achieved and all other existing functionalities are not broken. In the context of traditional verification, it basically asks for a complete and correct specification of the after-change network, which is not available in practice. 

Due to these two reasons, the full specification of exactly what a network should do is not available in practice. So using traditional network verification, which compares the changed network to a spec representing its expected behavior, is not possible. And yet engineers need a way to reliably make changes to such networks. They need to add, remove, or change functionality in a subpart of the network, typically while preserving most of the network's behavior.

\subsubsection{Manual diff inspection.}

\brief{Here is what engineers do in practice: they use differential analysis even though they have access to traditional verification.}

\begin{table*}
    \centering
    \begin{tabular}{|l|l|l|l|}
    \toprule
        Example packet of traffic class & Before-change paths & After-change paths & Inspection result \\ \midrule
        dstIP $ = 10.0.0.9$, ingress location = $DC_1$ & $\{DC_1 \rightarrow D \rightarrow A \rightarrow B \rightarrow C \rightarrow DC_3\}$ &  $\{DC_1 \rightarrow D \rightarrow drop \}$ & Expected\\ \midrule
        dstIP $ = 10.0.0.1$, ingress location = $DC_1$ & $\{DC_1 \rightarrow D \rightarrow A \rightarrow B \rightarrow DC_2\}$ &  $\{DC_1 \rightarrow D \rightarrow drop \}$ & Unexpected \\ 
    \bottomrule
    \end{tabular}
    \caption{The simplified change diff of the example change in \Cref{fig:dns}}
    \label{tab:change_diff}
\end{table*}

In practice, network operators have resorted to manual inspection of change ``diff'' to validate network changes even though they have access to verification tools. 
The workflow is generally as follows: 1) network engineers create a simulated/emulated replica of the network based on a recent snapshot and then 2) apply the change to the replica to derive the after-change network state.  
Next, 3) a dataplane simulator is used to compute the concrete forwarding paths of all traffic\footnote{Instead of considering all possible IP headers, network engineers usually consider only the traffic that is carried by the network. This information is provided by a network monitoring system based on NetFlow, which captures and stores the ingress interface and 5-tuple of all traffic as it enters the network.} in both the before-change and the after-change network. And finally, 4) the engineers manually inspect all classes of traffic whose forwarding paths are different in these two versions of the network, \IE, the ``diff'' of traffic path properties produced by the network change, to identify any unexpected bad behaviors. For example, the change diff for the example in \Cref{fig:dns} will contain two classes of traffic\footnote{This is a simplified change diff just to show case the idea. In reality, the number of traffic classes in this change diff will be much larger, as traffic may start from different routers inside $DC_1$ and thus has different paths.}, as shown in \Cref{tab:change_diff}. By auditing each class of changed traffic, the engineers will be able to identify that the first class is expected change impact and the second class is an unexpected bad behavior.

\brief{Our goal is to automate this process, making it less tedious and more rigorous.}

While this approach is more practical than maintaining a full specification of the network, it is still a tedious task. The number of traffic classes in a change diff usually falls in the range from O($10$) to O($10^5$), while the throughput of manual auditing is about O(10) classes per person per day even for expert engineers. We need an automated approach to help speed up this process. Moreover, while it is sufficient to ensure that no unexpected bad effect can happen by checking the change diff, it cannot ensure that all intended change impact is achieved. Some intended change impact may be missing from the change diff which is difficult to identify by just looking at the diff itself. We need to relate the entire before-change network to the entire after-change network to ensure that 1) all traffic that are intended to be changed are indeed changed in the expected way and meanwhile 2) all traffic that are intended to be preserved are not broken.

\subsubsection{Relational verification}

\brief{explain what relation verification is in general, in a similar style to the way in which we described traditional verification, with emphasis on what is different.  ie, in general a relational verification system demands a spec S2 that describes the relationship between old (Nold) and new (Nnew) networks and then checks that a pair of old and new networks meet that spec.  ie:
Nold, Nnew |= S2}

\brief{explain the pros:
1) incomplete information:  While network engineer is may not understand the totality of the network they are changing, They do understand the principle of preserving the functionality of any components they do not understand. In a relational system, one may succinctly specify that unknown components "stay the same" and thereby deal with the problem of incomplete information
2) scale:  while networks are vast, changes may often be small.  relational specifications usually scale not with the size of the network but with the size of the change, making such specifications tractable to write down and manage.  A system that automates the decision procedure Nold, Nnew |= S1 costs manual labor in terms of the size and complexity of S1 not Nold and Nnew.}

\begin{lstlisting}
spec dropForeign := {
    DC1-D  : preserve;
    .*-DC3  : drop;
} else {
    .*       : preserve;
}

\end{lstlisting}

\begin{figure*}
    \begin{subfigure}{.16\textwidth}  % Subfigure 1
        \centering
        \includegraphics[width=.99\textwidth]{figures/macro_example_preserve.png}
        \caption{preserve}
        \label{fig:macro_example_preserve}
    \end{subfigure}
    \begin{subfigure}{.16\textwidth}  % Subfigure 2
        \centering
        \includegraphics[width=.99\textwidth]{figures/macro_example_add.png}
        \caption{add}
        \label{fig:macro_example_add}
    \end{subfigure}
    \begin{subfigure}{.16\textwidth}  % Subfigure 3
        \centering
        \includegraphics[width=.99\textwidth]{figures/macro_example_remove.png}
        \caption{remove}
        \label{fig:macro_example_remove}
    \end{subfigure}
    \begin{subfigure}{.16\textwidth}  % Subfigure 4
        \centering
        \includegraphics[width=.99\textwidth]{figures/macro_example_replace.png}
        \caption{replace}
        \label{fig:macro_example_replace}
    \end{subfigure}
    \begin{subfigure}{.16\textwidth}  % Subfigure 5
        \centering
        \includegraphics[width=.99\textwidth]{figures/macro_example_drop.png}
        \caption{drop}
        \label{fig:macro_example_drop}
    \end{subfigure}
    \begin{subfigure}{.16\textwidth}  % Subfigure 6
        \centering
        \includegraphics[width=.99\textwidth]{figures/macro_example_any.png}
        \caption{any}
        \label{fig:macro_example_any}
    \end{subfigure}
    \caption{cap}
    \label{fig:macro_examples}
\end{figure*}

\begin{table*}
    \centering
    \begin{tabular}{|l|l|l|l|}
    \toprule
        Example packet of traffic class & Before-change paths & After-change paths & Inspection result \\ \midrule
        dstIP $ = 10.0.0.9$, ingress location = $DC_1$ & $\{DC_1 \rightarrow D \rightarrow A \rightarrow B \rightarrow C \rightarrow DC_3\}$ &  $\{DC_1 \rightarrow D \rightarrow drop \}$ & Expected\\ \midrule
        dstIP $ = 10.0.0.1$, ingress location = $DC_1$ & $\{DC_1 \rightarrow D \rightarrow A \rightarrow B \rightarrow DC_2\}$ &  $\{DC_1 \rightarrow D \rightarrow drop \}$ & Unexpected \\ 
    \bottomrule
    \end{tabular}
    \caption{The simplified change diff of the example change in \Cref{fig:dns}}
    \label{tab:change_diff}
\end{table*}

\begin{figure}
\centering
\begin{flushleft}
\begin{tikzpicture}[node distance = 1.5cm, on grid, auto]
\tikzstyle{every state}=[fill=white,draw=black,text=black,minimum size=15pt]
    \node (q0) [state, initial] {$q_0$};
    \node (q1) [state, accepting, right = of q0] {$q_1$};

    \path [->]
        (q0) edge node {a}   (q1);

    \node at (4.5,0) {FSA of $Prop$ expression $a$};
\end{tikzpicture}

\begin{tikzpicture}[node distance = 1.5cm, on grid, auto]
\tikzstyle{every state}=[fill=white,draw=black,text=black,minimum size=20pt]
    \node (q0) [state, initial] {$q_0$};
    \node (q1) [state, accepting, right = of q0] {$q_1$};

    \path [->]
        (q0) edge node {a:b}   (q1);

    \node at (4.5,0) {FST of $Rel$ expression $a \times b$};
\end{tikzpicture}
\end{flushleft}

    \caption{Simple examples of finite-state automata and finite-state transducers.}
    \label{fig:fsa_example}
\end{figure}

\begin{figure}
  %\centering
  \begin{bnf}(comment = {\#}, new-line-delim = {\|\|})[
    colspec={llcll},
    column{4}={font = \ttfamily},
  ]
    $t$  ::=
    || true          # true
    || !$t$          # negation
    || ($t_1$|$t_2$) # disjunction
    || $t_1$ \& $t_2$# conjunction
    || prefix = $x$  # prefix text
  \end{bnf}
  \caption{The extended syntax of \sysname FE.} 
  \label{fig:syntax_ext}
\end{figure}

\begin{table*}
    \centering
    \begin{tabular}{l|m{.6\textwidth}|m{.2\textwidth}}
        \toprule
        FE modifier & Description & RIR representation \\ \midrule
        \texttt{preserve} & All paths in the domain remain the same. & $\mathtt{I}(.^*)$\\ \midrule 
        \texttt{add($r$)} & All paths that match $r$ are added if not already present. All other paths in the domain remain the same. & $\mathtt{I}(.^*) ~|~ (.^* \times ~r)$ \\ \midrule
        \texttt{remove($r$)} & All paths in the domain that match $r$ are removed. All other paths in the domain remain the same. & $\mathtt{I}(~\overline{r}~)$ \\ \midrule
        \texttt{replace($r_1$,$r_2$)} & All paths in the domain that match $r_1$ are replaced by all paths that match $r_2$. All other paths in the domain (not matching $r_1$) remain the same. & $\mathtt{I}(~\overline{r_1}~) ~|~ (r_1 \times r_2)$\\ \midrule
        \texttt{drop} & All paths in the domain are replaced by a special path $drop$. & $.^* \times drop$\\ \midrule
        \texttt{any($r$)} & All paths in the domain and in $r$ are replaced by at least one path that matches $r$. & $.^* \times r$ (rewriting needed, see \Cref{sec:compilation})\\ \bottomrule
    \end{tabular}
    \vspace{5pt}
    \caption{The meaning of FE modifiers and their RIR representation. \xieyang{is the RIR column necessary?} \zak{I'd remove it}}
    \label{tab:modifiers}
\end{table*}

\subsubsection{Checking preservation with \sysname}
We then switched to validate that no unexpected bad changes happen to other parts of the network. We did so by adding an ``else'' clause to the previous spec:
\begin{lstlisting}
spec shiftBorderFull := 
    shiftBorder else {
    .* : preserve;
}
\end{lstlisting}
This additional clause means that all traffic that does not match the previous spec should have exactly the same set of forwarding paths before and after the change. And when checking the 4th implementation against this spec, we got \todo{xx} classes of violations which was surprising at first. Among them, network engineers discovered \todo{xx} classes of true positives. These are expected side effects of this change, albeit not considered by engineers beforehand. The rest of \todo{xx} classes are \textit{false positives} caused by defects in the underlying tool chain, \EG, due to a missing input route to the control plane simulator or a small part of configurations that are not yet supported by the simulator.

\subsubsection{Comparing \sysname with prior approaches.}
In terms of bug-finding ability, single-snapshot verification may fail to identify tricky bugs such as the one in \Cref{fig:shift_exit_v3}. Suppose users check two types of properties for this change. First, an end-to-end reachability that $S$ should be able to reach $D$ using some specific packet. Second, this traffic should go through $A1$ and should not go through $B1$ after change (\IE, waypointing properties). These properties will not flag the error in this case.

Manual diff inspection may also fail to identify some bugs when the intended change impact is not achieved, because such bugs leads to some entries to be missing from the diff, such as in \Cref{fig:shift_exit_v1}. In industrial settings, a change diff usually has a long list of entries consisting of intended changes, unexpected changes, and false positives. Therefore, users looking at the diff may fail to recognize the missing intended change, especially when only a part of the intended change is missing.

In terms of the efficiency to debug network changes, manual diff inspection often reports a much longer list of traffic class that needs to be inspected. In the change above, there was an average of \todo{xxx} changing traffic classes to be inspected in validating the 4 versions of implementation. When validating changes using \sysname, as demonstrated above, engineers are able to focus on one goal at a time. The number of counterexamples that need to be inspected for checking productivity were \todo{xx}, \todo{xx} and \todo{xx} respectively for the three buggy versions. And in checking preservation, engineers inspected \todo{xx} classes only once. Using \sysname is more efficient. Indeed, the manual diff inspect of the four versions took the team 4 weeks, while using \sysname is can be done in a course of hours.
